Llamarine: Open-source Maritime Industry-specific Large Language Model

Large Language Models (LLMs) have demonstrated substantial potential in addressing complex reasoning tasks, yet their general-purpose nature often limits their effectiveness in specialized domains such as maritime navigation. To bridge this gap, we introduce Llamarine, the first open-source LLM designed specifically for maritime navigation. Llamarine 1.0 is developed through continued pretraining and fine-tuning on a high-quality corpus comprising maritime textbooks, research publications, and web text from Wikipedia. This domain-specific training enables the model to acquire expert-level knowledge in navigational principles, collision avoidance, route optimization, and regulatory compliance. Our key contributions include (a) the curation of a comprehensive maritime dataset from authoritative sources, ensuring depth and reliability in the model's knowledge base; (b) the development of a foundational model capable of reasoning about complex navigational challenges with greater accuracy than general-purpose LLMs; and (c) the establishment of a benchmark to evaluate performance in maritime-specific decision-making tasks. Experimental results demonstrate that Llamarine outperforms both general-purpose and commercial LLMs in critical navigation-related tasks, such as trajectory planning, risk assessment, and compliance with maritime regulations. By providing an open-source foundation model trained exclusively on high-quality maritime literature, Llamarine paves the way for AI-driven advancements in maritime safety, efficiency, and operational decision-making.

==> data_en.tex <==
\usepackage{color}
	
%%Title: 
\title{Llamarine: Open-source Maritime Industry-specific Large Language Model}

%%Contact address: 
\address{Name, Affiliation, Address, Phone number, Facsimile number, and E-mail address}

%%Name of authors:
\author{%
The Program Committee of the JSAI20XX\first
\and
Second Author's Name\second
}

%%Affiliations:
\affiliate{
\first{} The Japanese Society for Artificial Intelligence
\and
\second{} Affiliation \#2
}

%%
%\Vol{28}        %% <-- 25
%\session{0A0-00}%% <-- ID

\begin{abstract}
Here is an abstract of up to 150 words in English or 300 characters in Japanese. 
This document describes the formatting guidelines for English manuscripts in \LaTeX{} of the annual conference of JSAI. This is also a sample of a formatted manuscript (see 2.4 for writing the abstract).
\end{abstract}

%\setcounter{page}{1}
\def\Style{``jsaiac.sty''}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em%
 T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\def\JBibTeX{\leavevmode\lower .6ex\hbox{J}\kern-0.15em\BibTeX}
\def\LaTeXe{\LaTeX\kern.15em2$_{\textstyle\varepsilon}$}

\begin{document}
\maketitle

\section{Introduction}

This article contains format guidelines for authors contributing to JSAI 20XX using \LaTeX{}. The conference proceedings will be distributed on a conference Web site containing PDF files prepared by the authors. To ensure that all papers in the proceedings have a uniform appearance, please refer to the following instructions. \textcolor{red}{This information may be updated even after it is released. Please confirm that it is the latest version before your submission.}


\section{General Information}
\subsection{File format and size}

The manuscript file should be an Adobe(R) PDF (Portable Document Format) file. The size of the manuscript file should be less than 3 Mbytes. The extension of the file name should be ``.pdf".

\subsection{Header}

The conference name in the header and your paper ID should not be included, because the organizing committee will add them.

\subsection{Title and author's name(s)}

The title of the paper and author's name(s) should be the same as those appeared in the application form. \textcolor{red}{Please ensure there are no differences between title and author's name(s) in the manuscript and presentation application.}

\subsection{Abstract}

Please include (1) the objective and (2) the outline of the conclusions of your results in the abstract under the author information. Also, please state the outline of your method as necessary in the abstract.  \textcolor{red}{Submissions without any description regarding (1) or (2) in the abstract may not be considered for presentation or publication.}

\subsection{Paper length}

The length of each paper is two pages on A4 size paper. Up to two additional pages are accepted.

\subsection{International session}

English is the only acceptable language for the international sessions. Papers for the international sessions will be included on the conference Web site, from which papers that match the general requirements of relevance and scientific and technological excellence are encouraged to submit to the Journal of New Generation Computing.

\section{Style file for \LaTeX{}}

When you use the style file for JSAI20XX named ``jsaiac.sty'', please specify a style option as follows;

For \LaTeX{}2.09, 
\begin{verbatim}
\documentstyle[twocolumn,jsaiac]{article}
\end{verbatim}

For \LaTeXe{}, 
\begin{verbatim}
\documentclass[twocolumn]{article}
\usepackage{jsaiac}
\end{verbatim}


\def\Label{\vskip.5\baselineskip\noindent$\circ$\hskip3pt{}}

\Label The first page: 
Please use the following commands;
\begin{itemize}
\item Title: 
\begin{verbatim}
\title{Title of your paper}
\end{verbatim}

\item Name of authors:
\begin{verbatim}
\author{%
   Name of the first author\first{}
\and
   Name of the second author\second{}
}
\end{verbatim}

If the affiliations of authors are different, please use the following commands;

\begin{verbatim}
\def\first{\hbox{$\m@th^{\ast 1}$\hss}}
\def\second{\hbox{$\m@th^{\ast 2}$\hss}}
\def\third{\hbox{$\m@th^{\ast 3}$\hss}}
\def\fourth{\hbox{$\m@th^{\ast 4}$\hss}}
\def\fifth{\hbox{$\m@th^{\ast 5}$\hss}}
\def\sixth{\hbox{$\m@th^{\ast 6}$\hss}}
\def\seventh{\hbox{$\m@th^{\ast 7}$\hss}}
\def\eighth{\hbox{$\m@th^{\ast 8}$\hss}}
\def\ninth{\hbox{$\m@th^{\ast 9}$\hss}}
\end{verbatim}

You should add the same commands for corresponding affiliations. 
If there is only one affiliation, the \verb|\first| is not needed.

\item Affiliations: 
\begin{verbatim}
\affiliate{
   \first{}Affiliation #1
\and
   \second{}Affiliation #2
\and
   \third{}Affiliation #3
}
\end{verbatim}

\item Contact address: 
Use the \verb|\address| command as follows;

\begin{verbatim}
\address{name, affiliation, address, 
phone number, Fax number, 
e-mail address}
\end{verbatim}
\end{itemize}

\Label Misc.
\begin{itemize}
\item References: The style of the Journal of JSAI is preferred.
Some samples are shown below.

\end{itemize}

\begin{thebibliography}{99}
\bibitem[Knuth 84]{texbook}
 Knuth,~D.~E.: The \TeX{}book, Addison-Wesley (1984),
\bibitem[Lamport 86]{latexbook}
Leslie,~L: \LaTeX{}: {A} Document Preparation System (Updated for
  \LaTeX{}2$\varepsilon$), Addison-Wesley, 2nd edition (1998)
\end{thebibliography}
%%












